Developers Need Protection, Too: Perspectives and Research Challenges for Privacy in Social Coding Platforms

Social Coding Platforms (SCPs) like GitHub have become central to modern software engineering thanks to their collaborative and version-control features. Like in mainstream Online Social Networks (OSNs) such as Facebook, users of SCPs are subjected to privacy attacks and threats given the high amounts of personal and project-related data available in their profiles and software repositories. However, unlike in OSNs, the privacy concerns and practices of SCP users have not been extensively explored nor documented in the current literature. In this work, we present the preliminary results of an online survey (N=105) addressing developers' concerns and perceptions about privacy threats steaming from SCPs. Our results suggest that, although users express concern about social and organisational privacy threats, they often feel safe sharing personal and project-related information on these platforms. Moreover, attacks targeting the inference of sensitive attributes are considered more likely than those seeking to re-identify source-code contributors. Based on these findings, we propose a set of recommendations for future investigations addressing privacy and identity management in SCPs.

==> CHASE 2023/drafts.tex <==
INTRO:

Yet, such actions can have great financial, 

that such cases of secret sprawl in corporate repositories have increased significantly /account for  ... All in all, it only takes a ``developer inadvertently pushing to a public repository while thinking working on a private environment is enough'' Hence, this becomes a perfect playground for malicious users. Altogether, profile information, code and ML FACILITATE such attacks ...Plus the inference capabilities of advanced ML models .

 Our data show
shows that the extent of publicly-exposed secrets on GitHub has more than doubled since 2020. 

account for...

Hence, loose privacy practices in SCPs can have consequences beyond the 



``In the case of Samsung, the cybercriminals claim to have \textbf{stolen 190 Gb of data} and the tech giant has confirmed that the compromised information included source code related to Galaxy devices.''
``In many cases they appear to have obtained source code belonging to the victims, some of which has been made public.''

`` let’s not forget that mistakes do happen more often than we please to think and without making a noise: a developer inadvertently pushing to a public repository while thinking working on a private environment is enough.''

Hence, unlike in traditional OSNs, loose privacy practices and a lack of awareness in SCPs can have consequences that go beyond the

shallow

a developer working at Samsung inadvertently pushed thousands of secret keys into a public repository  

 \textbf{secrets sprawl in corporate repositories}

All in all, it took just one clumsy developer . Therefore, poor privacy practices in SCPs can have consequences that go beyond one individual....

thousands of secrets keys  .. It has been repeatedly reported: leaked passwords used thereafter in social engineering attacks. This speaks about the lack of awareness of the developers .... Take a proactive atitude towards the privacy in SCPs.

(let us consider GitHub as a representative case...)

Information that could be used in a potential Social Engineering attack

%Still, up to our knowledge, the privacy of SCP users has not received as much attention as that of OSNs. 

%Considering the increasing popularity and the supporting role of these platforms for 

%Considering the increasing popularity and importance of these platforms for the software engineering community nowadays, it is fundamental to further investigate this aspect 

%However, recent advances in ML models and systems have become a ``double-edged sword'' in the quest for privacy as they can be used for both counteracting and crafting ML-enabled privacy attacks.

------------------------------------
The overarching goal of this project is to delve into the anatomy of ML-based privacy attacks in SCPs. Particularly, it seeks to identify the conditions under which these attacks could be performed and elaborate PETs to protect developers’ digital identity. That is, privacy tools and mechanisms for supporting their regular activities within SCPs (e.g., push, edit, or review software projects) while minimizing the risks related to re-identification, inference, and linkability. For this, it is critical to thoroughly understand not only the technical aspects of ML-based privacy attacks but also developers’ privacy goals and expectations. Hence, we plan to elaborate on the next Research Questions (RQs) following an interdisciplinary approach:

\textbf{RQ1: How can ML-based privacy attacks be performed within SCPs?}

As mentioned earlier, users of SCPs reveal large amounts of data (either directly or indirectly) inside their profiles and as a consequence of their online interactions. Prior research in OSNs has shown how ML-based attacks can leverage such data to infer sensitive attributes and re-identify individuals. Therefore, we plan to investigate how these attacks can be executed and tailored to the resources available in SCPs (e.g., data from profiles, commits, and reports). 

\textbf{RQ2: How aware are the users of SCPs about these attacks and their privacy impact? }

To empower users of SCPs with PETs aiming to protect their digital identities, it is important to understand their privacy concerns and practices. That is, up to what extent they are aware of the possibility of becoming targets of ML-based privacy attacks and whether they take proactive measures to avoid such attacks. Hence, we plan to conduct empirical studies to gather insights in this regard and use them thereafter to elaborate PETs with a strong usability focus.

\textbf{RQ3: Which countermeasures can be envisaged to protect users against these attacks?}

Countermeasures aim to mitigate (or even eradicate) the risks of ML-based privacy attacks. Adversarial examples are a promising approach capable of fooling sensitive-attribute classifiers and other inference models alike. Still, such examples should satisfy certain utility-loss constraints, which may vary across contexts and application domains. Therefore, we will investigate how to craft effective adversarial examples while preserving the utility of SDP datasets. Particularly, we will investigate what type of noise can be added to SDP data in order to meet the individual and collective privacy/utility goals of SDP users.

\textbf{RQ4: How can these mechanisms be translated into identity management PETs for SCPs?}

The usability of the generated countermeasures is an important aspect that must be explicitly considered. It has been extensively argued throughout the privacy literature that PETs often fail to meet users’ expectations for several reasons. These include a one-size-fits-all design, an unfriendly interface, and wrongly-elicited requirements. Hence, we plan to outline and evaluate different integration alternatives for the envisaged countermeasures within mainstream SDPs. 

To answer these RQs we will apply different methods and tools from different disciplines, including computer science and social psychology. Particularly, we foresee the use of data mining techniques for the generation of datasets, DL algorithms to train and test the aforementioned attack models, and questionnaires/surveys to conduct empirical research on privacy in SCPs.

\section{Directions for Future Research}

All in all, prior work has explored the uses of advanced ML methods for (i) finding correlations between developers’ activities in SCPs and their demographic characteristics and (ii) re-identify source code contributors through stylistic coding patterns. Still, specific ML-based privacy attacks targeting SCP users have not been thoroughly investigated nor documented in the current literature. Moreover, to the extent of our knowledge, no specific countermeasures have been yet proposed to resist these attacks.

-------------------------------------
In principle, pull-based development can help mitigating this issue thanks to 


Although applying a pull-based development framework can initially contribute  


Given the collaborative nature of SCPs, such conflicts can easily arise, for instance, when developers disclose secrets or introduce code vulnerabilities in shared repositories. Current pull-based development frameworks can be considered as powerful instruments against these social threats as they 


contribute to a shared repository; for instance, by sharing secrets or pushing insecure code that can ultimately compromise the security and privacy of the whole team.




The pull request mechanism implemented in SCPs can be seen as a

Because of their collaborative nature, conflicts of this type can easily arise as well in SCPs when contributing to a in a shared repository.


pushing code the visibility of a common repository, or sharing secrets without others' consent. Hence, it would be worthwhile to investigate the privacy threats arising from users' conflicting privacy goals in SCPs and elaborate computational mechanisms for their effective resolution.

or even assess how robust the current SCP mechanisms are against this particular type of conflicts (e.g., pull requests).

the relationship between these concerns and the adoption of pull requests

==> drafts.tex <==
INTRO:

Yet, such actions can have great financial, 

that such cases of secret sprawl in corporate repositories have increased significantly /account for  ... All in all, it only takes a ``developer inadvertently pushing to a public repository while thinking working on a private environment is enough'' Hence, this becomes a perfect playground for malicious users. Altogether, profile information, code and ML FACILITATE such attacks ...Plus the inference capabilities of advanced ML models .

 Our data show
shows that the extent of publicly-exposed secrets on GitHub has more than doubled since 2020. 

account for...

Hence, loose privacy practices in SCPs can have consequences beyond the 



``In the case of Samsung, the cybercriminals claim to have \textbf{stolen 190 Gb of data} and the tech giant has confirmed that the compromised information included source code related to Galaxy devices.''
``In many cases they appear to have obtained source code belonging to the victims, some of which has been made public.''

`` let’s not forget that mistakes do happen more often than we please to think and without making a noise: a developer inadvertently pushing to a public repository while thinking working on a private environment is enough.''

Hence, unlike in traditional OSNs, loose privacy practices and a lack of awareness in SCPs can have consequences that go beyond the

shallow

a developer working at Samsung inadvertently pushed thousands of secret keys into a public repository  

 \textbf{secrets sprawl in corporate repositories}

All in all, it took just one clumsy developer . Therefore, poor privacy practices in SCPs can have consequences that go beyond one individual....

thousands of secrets keys  .. It has been repeatedly reported: leaked passwords used thereafter in social engineering attacks. This speaks about the lack of awareness of the developers .... Take a proactive atitude towards the privacy in SCPs.

(let us consider GitHub as a representative case...)

Information that could be used in a potential Social Engineering attack

%Still, up to our knowledge, the privacy of SCP users has not received as much attention as that of OSNs. 

%Considering the increasing popularity and the supporting role of these platforms for 

%Considering the increasing popularity and importance of these platforms for the software engineering community nowadays, it is fundamental to further investigate this aspect 

%However, recent advances in ML models and systems have become a ``double-edged sword'' in the quest for privacy as they can be used for both counteracting and crafting ML-enabled privacy attacks.

------------------------------------
The overarching goal of this project is to delve into the anatomy of ML-based privacy attacks in SCPs. Particularly, it seeks to identify the conditions under which these attacks could be performed and elaborate PETs to protect developers’ digital identity. That is, privacy tools and mechanisms for supporting their regular activities within SCPs (e.g., push, edit, or review software projects) while minimizing the risks related to re-identification, inference, and linkability. For this, it is critical to thoroughly understand not only the technical aspects of ML-based privacy attacks but also developers’ privacy goals and expectations. Hence, we plan to elaborate on the next Research Questions (RQs) following an interdisciplinary approach:

\textbf{RQ1: How can ML-based privacy attacks be performed within SCPs?}

As mentioned earlier, users of SCPs reveal large amounts of data (either directly or indirectly) inside their profiles and as a consequence of their online interactions. Prior research in OSNs has shown how ML-based attacks can leverage such data to infer sensitive attributes and re-identify individuals. Therefore, we plan to investigate how these attacks can be executed and tailored to the resources available in SCPs (e.g., data from profiles, commits, and reports). 

\textbf{RQ2: How aware are the users of SCPs about these attacks and their privacy impact? }

To empower users of SCPs with PETs aiming to protect their digital identities, it is important to understand their privacy concerns and practices. That is, up to what extent they are aware of the possibility of becoming targets of ML-based privacy attacks and whether they take proactive measures to avoid such attacks. Hence, we plan to conduct empirical studies to gather insights in this regard and use them thereafter to elaborate PETs with a strong usability focus.

\textbf{RQ3: Which countermeasures can be envisaged to protect users against these attacks?}

Countermeasures aim to mitigate (or even eradicate) the risks of ML-based privacy attacks. Adversarial examples are a promising approach capable of fooling sensitive-attribute classifiers and other inference models alike. Still, such examples should satisfy certain utility-loss constraints, which may vary across contexts and application domains. Therefore, we will investigate how to craft effective adversarial examples while preserving the utility of SDP datasets. Particularly, we will investigate what type of noise can be added to SDP data in order to meet the individual and collective privacy/utility goals of SDP users.

\textbf{RQ4: How can these mechanisms be translated into identity management PETs for SCPs?}

The usability of the generated countermeasures is an important aspect that must be explicitly considered. It has been extensively argued throughout the privacy literature that PETs often fail to meet users’ expectations for several reasons. These include a one-size-fits-all design, an unfriendly interface, and wrongly-elicited requirements. Hence, we plan to outline and evaluate different integration alternatives for the envisaged countermeasures within mainstream SDPs. 

To answer these RQs we will apply different methods and tools from different disciplines, including computer science and social psychology. Particularly, we foresee the use of data mining techniques for the generation of datasets, DL algorithms to train and test the aforementioned attack models, and questionnaires/surveys to conduct empirical research on privacy in SCPs.

\section{Directions for Future Research}

All in all, prior work has explored the uses of advanced ML methods for (i) finding correlations between developers’ activities in SCPs and their demographic characteristics and (ii) re-identify source code contributors through stylistic coding patterns. Still, specific ML-based privacy attacks targeting SCP users have not been thoroughly investigated nor documented in the current literature. Moreover, to the extent of our knowledge, no specific countermeasures have been yet proposed to resist these attacks.

-------------------------------------
In principle, pull-based development can help mitigating this issue thanks to 


Although applying a pull-based development framework can initially contribute  


Given the collaborative nature of SCPs, such conflicts can easily arise, for instance, when developers disclose secrets or introduce code vulnerabilities in shared repositories. Current pull-based development frameworks can be considered as powerful instruments against these social threats as they 


contribute to a shared repository; for instance, by sharing secrets or pushing insecure code that can ultimately compromise the security and privacy of the whole team.




The pull request mechanism implemented in SCPs can be seen as a

Because of their collaborative nature, conflicts of this type can easily arise as well in SCPs when contributing to a in a shared repository.


pushing code the visibility of a common repository, or sharing secrets without others' consent. Hence, it would be worthwhile to investigate the privacy threats arising from users' conflicting privacy goals in SCPs and elaborate computational mechanisms for their effective resolution.

or even assess how robust the current SCP mechanisms are against this particular type of conflicts (e.g., pull requests).

the relationship between these concerns and the adoption of pull requests
